Ethosight: A Reasoning-Guided Iterative Learning System for Nuanced Perception based on Joint-Embedding & Contextual Label Affinity

Traditional computer vision models often necessitate extensive data acquisition, annotation, and validation. These models frequently struggle in real-world applications, resulting in high false positive and negative rates, and exhibit poor adaptability to new scenarios, often requiring costly retraining. To address these issues, we present Ethosight, a flexible and adaptable zero-shot video analytics system. Ethosight begins from a clean slate based on user-defined video analytics, specified through natural language or keywords, and leverages joint embedding models and reasoning mechanisms informed by ontologies such as WordNet and ConceptNet. Ethosight operates effectively on low-cost edge devices and supports enhanced runtime adaptation, thereby offering a new approach to continuous learning without catastrophic forgetting. We provide empirical validation of Ethosight's promising effectiveness across diverse and complex use cases, while highlighting areas for further improvement. A significant contribution of this work is the release of all source code and datasets to enable full reproducibility and to foster further innovation in both the research and commercial domains.

==> diagrams/backupfig1.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[
  node distance = 10mm and 5mm,
  block/.style = {draw, rectangle, minimum width=20mm, minimum height=10mm, align=center},
  arrow/.style = {->, >=stealth},
  dashline/.style = {draw, dashed}
]

\node[block] (deepvision) {DeepVision Video\\ Frame Stream};
\node[block, below=of deepvision, yshift=-2mm] (input) {User Input /\\ Use Case Definition\\ (in natural language)};
\node[block, below=of input] (label) {Reasoning-Based\\ Generation of\\ Initial Labels};
\node[block, below=of label] (embedding) {Label Affinity Calculation};
\node[draw, diamond, aspect=2, below=of embedding] (decision) {Convergence?};
\node[block, below=of decision] (output) {Deep Scene Analysis};
\node[block, dashed, below=of output] (optional) {Optional: Natural Language Output /\\API Calls};
\node[block, below=of optional, yshift=-1mm] (analytics) {Deep Vision Ethosight\\ Analytics Stream};

\draw [arrow] (input) -- (label);
\draw [arrow] (label) -- (embedding);
\draw [arrow] (embedding) -- (decision);
\draw [arrow] (decision) -- node[left] {Yes} (output);
\draw [arrow] (decision) -- node[above] {No} ++(-2.2,0) |- (label);
\draw [arrow] (deepvision.east) -- ++(1.2,0) -- ([xshift=12mm]deepvision.east|-embedding.north) -- (embedding);
\draw [arrow] (output) -- (optional);
\draw [arrow] (optional) -- (analytics);

\node[draw, fit=(input) (label) (embedding) (decision) (output) (optional), inner xsep=10mm, label=above:{Ethosight Iterative Learning Loop}] {};

\end{tikzpicture}

\caption{Overview of the Ethosight system, which processes streaming video input from DeepVision through an iterative learning loop. The loop involves reasoning-based generation of initial labels, label affinity calculation, and assessment of convergence. If convergence is achieved, deep scene analysis is performed and optional further actions such as reasoning and natural language generation (NLG) or API calls are taken. The results are then passed back into the DeepVision Ethosight Analytics Stream.}
\label{fig:ethosight_system}
\end{figure}


==> sections/DeepVisionOverview.tex <==
\section{Open Source Implementation and Scalable Analytics Framework}
Ethosight is an integral part of Deep Vision \cite{DeepVision}, an open-source, serverless edge platform designed to address explainable perception challenges. Deep Vision is principally focused on advancing the development and deployment of innovative computer vision and multimodal spatiotemporal algorithms. This scalable analytics framework is designed to provide solutions to several key issues in the field, such as improving analytics accuracy on spatio-temporal data, self-supervised learning, lifelong learning, and creating explainable models.

Deep Vision, and by extension Ethosight, is architected to run in any environment that supports GPU and Docker (including the NVIDIA extension). 

The implementation of Deep Vision is open-source, making it accessible for further development and modifications by the community. The system is versatile and scalable, allowing for seamless integration of additional sensor types, viewing analytics on various dashboards, and enabling users to receive alerts through SMS or emails.

Getting Started with Deep Vision:

For those interested in exploring, experimenting with, or contributing to the development of Deep Vision, the detailed instructions for getting started can be found at our GitHub repository [Insert Link Here].

This repository includes a guide to setting up and running Deep Vision, along with the complete codebase for Ethosight. Users can not only understand the inner workings of Ethosight and Deep Vision but also modify and customize it to suit their specific requirements.

Our aim with this open-source implementation is to stimulate further research and development in the field of computer vision and multimodal spatio-temporal algorithms, and we invite the broader community to join us in this endeavour.



==> sections/ExperimentsAndResults_backup.tex <==
\section{Experiments and Results}

The efficacy of Ethosight was evaluated through a series of experiments structured into three critical phases. These stages map the system's lifecycle: system bootstrapping, deployment with GPU access, and deployment without GPU access. The focus was on Ethosight's capacity to accurately identify subtle behaviors and events.

\subsection{Phase 1: System Bootstrapping}

In the bootstrapping phase, Ethosight begins with zero prior symbolic knowledge. The system is presented with a user-given initial prompt: "we are targeting video analytics systems for people and animals in public spaces of all types including retail, education, residential, and businesses. Our primary interest is relating to health, safety, and security. If any person or animal is in any kind of danger or requires assistance, this is the highest priority."

The main aim during this phase is to allow Ethosight to generate an initial set of labels pertinent to the user's needs, employing the GPT-4 based iterative reasoning loop. This creation of labels is a function of the given prompt and the context in which Ethosight operates, steering clear of any manual or hand-crafted labels.

Given the wide-ranging requirements of the system (spanning public spaces such as retail, education, residential, and businesses), the system's initial dataset is potentially broad and varied, focusing on aspects relating to health, safety, and security for both humans and animals.

This phase involves high GPU load due to the computation of potentially hundreds or thousands of relevant label embeddings based on the initial prompt. Despite the high computational demands, the bootstrapping phase is crucial in setting the stage for Ethosight's autonomous learning and subsequent operation. Due to the computational intensity, this phase may not run in real-time, but it sets the foundation for Ethosight's knowledge base that will be critical in subsequent phases.

The label affinity scores, computed via a multimodal embedding process, act as the initial knowledge base, which Ethosight will continually refine and build upon in the next phases of deployment.

\subsection{Phase 2: Deployment with GPU Access}

During the second phase, Ethosight is deployed within an environment that affords access to 5GB or more of GPU memory. This allows the system to leverage its iterative learning loop that is not only able to continuously incorporate new labels into its knowledge base but also adaptable to various types of reasoners and knowledge bases. Ethosight's iterative learning process is designed to be versatile and can work with different AI systems including, but not limited to, semantic knowledge bases like WordNet and symbolic reasoning engines such as OpenNARS.

This versatility underscores Ethosight's capability to function efficiently even in the absence of large-scale AI models like GPT-4. This potentially allows for the use of smaller, open-source models, thereby widening the range of deployment scenarios, reducing required computational resources, and increasing Ethosight's accessibility.

In parallel, the system refines its contextual analytics while performing real-time analytics. This ability to learn on the go and adapt its knowledge base without the need for a human-in-the-loop, while also providing the option for human intervention, is a major strength. Furthermore, the learnings and insights generated in this GPU-enabled environment can be directly transferred to no-GPU environments, highlighting Ethosight's scalable and flexible nature.

In this phase, we conducted further experiments to test Ethosight's real-time performance and its ability to use its iterative learning capabilities in detecting complex real-time events. This was key to understanding Ethosight's operational readiness and its capacity to function in diverse real-world situations.

\subsection{Phase 3: Deployment without GPU Access}

In the final phase, Ethosight operates in a non-GPU environment. Here, all label embeddings are precomputed, which circumvents the need for active, iterative learning via reasoning. However, Ethosight effectively leverages its previously acquired knowledge, operating solely on CPU power.

Throughout all phases and deployments, Ethosight exercises an implementation of Alfred Korzybski's "time-binding" concept, often used to depict the human ability to accumulate and transmit knowledge across generations. In the context of Ethosight, this machine implementation of "time-binding" enables the transfer and utilization of learnings and symbolic knowledge from one computational environment to another, irrespective of whether these environments are GPU- or CPU-powered. As such, Ethosight exhibits a form of generational learning, thereby representing the property of time-binding in machines.

The significant advantage of this mode is the enablement of edge intelligence, allowing Ethosight to efficiently function within environments constrained by computational resources, thereby substantially broadening its range of application.

Experiments in this phase aimed to assess Ethosight's operational effectiveness in a CPU-only, resource-constrained setting, and its capacity to utilize pre-existing symbolic knowledge efficiently. The outcomes of these tests emphasized Ethosight's potential to push the boundaries of AI by integrating aspects of generational learning, emulating human intelligence.

\section{Discussion}

Our series of experiments, spanning the three critical phases of Ethosight's development, have illuminated its progress from an initial bootstrapping phase - bereft of any pre-existing symbolic knowledge - to full-fledged deployment in GPU-enabled and non-GPU environments.

This AI system's flexibility is a testament to its underlying design, permitting the effortless transfer of symbolic knowledge and learnings from one computational environment to another, irrespective of the presence of a GPU. This capability not only exemplifies the machine implementation of Korzybski's "time-binding" concept, but also facilitates edge intelligence, making Ethosight a viable solution for resource-constrained environments.

In the following sections, we delve into the detailed results of each phase. We will discuss Ethosight's performance and iterative learning capacity in accurately identifying complex events such as shoplifting, child endangerment, and medical emergencies, thereby highlighting its potential to reshape the landscape of real-time video analytics. 

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{images/shoplifting.png}
\caption{Shoplifting event detected by Ethosight.}
\label{fig:shoplifting_event}
\end{figure}

%\FloatBarrier

\begin{table}[h]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Label} & \textbf{Affinity Score} \\ 
\hline
shoplifting & 0.9334480166435242 \\ 
\hline
suspicious behavior & 0.02523977681994438 \\ 
\hline
loitering & 0.011876602657139301 \\ 
\hline
man & 0.005518920719623566 \\ 
\hline
bagging items & 0.005208194721490145 \\ 
\hline
commuting & 0.0046491436660289764 \\ 
\hline
pickpocketing & 0.003923620563000441 \\ 
\hline
employee theft & 0.0013351356610655785 \\ 
\hline
burglary & 0.0008288859971798956 \\ 
\hline
returning items & 0.0007222711574286222 \\ 
\hline
browsing & 0.0006676515331491828 \\ 
\hline
mall & 0.0005949098849669099 \\ 
\hline
stalking & 0.0005586156621575356 \\ 
\hline
shopping & 0.00036094742245040834 \\ 
\hline
passenger & 0.00032686968916095793 \\ 
\hline
pedestrian & 0.0003050807863473892 \\ 
\hline
sales associate & 0.00025447510415688157 \\ 
\hline
trying on clothes & 0.00023706437787041068 \\ 
\hline
\end{tabular}
\caption{Shoplifting Event Labels and Affinity Scores}
\label{table:1}
\end{table}

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{images/kitchenaccident.png}
\caption{Dangerous kitchen event detected by Ethosight.}
\label{fig:kitchenaccident_event}
\end{figure}

%\FloatBarrier

\begin{table}[h]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Label} & \textbf{Affinity Score} \\ 
\hline
child in danger & 0.4346351623535156 \\ 
\hline
cooking & 0.26900413632392883 \\ 
\hline
burglary & 0.0736141949892044 \\ 
\hline
fire\_prevention & 0.07326945662498474 \\ 
\hline
gas\_leak\_detection & 0.06314415484666824 \\ 
\hline
repairing & 0.017247511073946953 \\ 
\hline
vomiting & 0.008393174037337303 \\ 
\hline
fire\_safety & 0.0065605794079601765 \\ 
\hline
decorating & 0.006369316019117832 \\ 
\hline
buying & 0.0054978723637759686 \\ 
\hline
peeping tom & 0.004484186880290508 \\ 
\hline
fire\_investigation & 0.0030823920387774706 \\ 
\hline
child abuse & 0.0020500756800174713 \\ 
\hline
oven & 0.0017948184395208955 \\ 
\hline
monitor & 0.0016760976286605 \\ 
\hline
\end{tabular}
\caption{Kitchen Event Labels and Affinity Scores}
\label{table:2}
\end{table}

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{images/poisonrisk.png}
\caption{Poisoning risk event detected by Ethosight.}
\label{fig:poisonrisk_event}
\end{figure}

%\FloatBarrier

\begin{table}[h]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Label} & \textbf{Affinity Score} \\ 
\hline
poisoning risk & 0.5816919207572937 \\ 
\hline
cleaning & 0.16239871084690094 \\ 
\hline
chemical spill & 0.12470459192991257 \\ 
\hline
poisoning & 0.046840012073516846 \\ 
\hline
chemicals & 0.034766871482133865 \\ 
\hline
child in danger & 0.011968997307121754 \\ 
\hline
vomiting & 0.005567247048020363 \\ 
\hline
presenting & 0.005016577895730734 \\ 
\hline
suspicious behavior & 0.005008356180042028 \\ 
\hline
chemical hazard & 0.004292265512049198 \\ 
\hline
baby & 0.0033497000113129616 \\ 
\hline
chemical weapon & 0.002891452284529805 \\ 
\hline
carbon\_monoxide\_poisoning & 0.0012668760027736425 \\ 
\hline
child abuse & 0.0007986582349985838 \\ 
\hline
threatening & 0.0006131484406068921 \\ 
\hline
\end{tabular}
\caption{Poison Risk Event Labels and Affinity Scores}
\label{table:3}
\end{table}

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{images/fight.png}
\caption{Fight detected by Ethosight.}
\label{fig:fight_event}
\end{figure}

%\FloatBarrier

\begin{table}[h]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Label} & \textbf{Affinity Score} \\ 
\hline
fighting & 0.4580756723880768 \\ 
\hline
violence & 0.3671010136604309 \\ 
\hline
animal bite & 0.10481132566928864 \\ 
\hline
violent gestures & 0.021410921588540077 \\ 
\hline
threatening & 0.012375416234135628 \\ 
\hline
riot & 0.006673006806522608 \\ 
\hline
stun gun & 0.004463140852749348 \\ 
\hline
posing & 0.003417507978156209 \\ 
\hline
brass knuckles & 0.003205067478120327 \\ 
\hline
throwing objects & 0.0025822892785072327 \\ 
\hline
meeting & 0.0016013321001082659 \\ 
\hline
pushing & 0.0013757663546130061 \\ 
\hline
pepper spray & 0.0011946778977289796 \\ 
\hline
hitting & 0.0010379304876551032 \\ 
\hline
harassment & 0.0009538165759295225 \\ 
\hline
\end{tabular}
\caption{Fight Event Labels and Affinity Scores}
\label{table:4}
\end{table}

\subsection{Benchmarking}

This is TBD. Kinect 400 dataset may be used. Currently researching datasets for more difficult to train use cases such as "person in danger" etc... From an analytics perspective, the real power of Ethosight lies in accurate analytics for difficult to train and expressly define events.

==> sections/ExperimentsAndResults_backup2.tex <==
\section{Experiments and Results}
\subsection{Multi-class Classification Accuracy}

\subsubsection{Objective of the Multi-class Classification Test}
The objective of this test was to evaluate how well the Ethosight model can distinguish between 13 different anomaly classes and 1 ``normal event'' class using the UCF Crime dataset.

\subsubsection{Model Used}
Our model is an Ethosight zero-shot application. It starts from a blank slate with no pre-trained knowledge other than the 14 ground truth labels. The underlying joint embedding technique used for this model is ImageBind.

\subsubsection{Preprocessing and Feature Engineering}
\begin{itemize}
    \item No preprocessing steps are applied to the image data. Images are used as-is without normalization, data augmentation, or handling of missing or corrupted data.
    \item The underlying joint embedding used by Ethosight, in this case ImageBind, effectively captures subtle features in the image data.
    \item The label-to-affinity scores generated by Ethosight are critical in the model's sensitivity to these subtle features.
    \item These scores allow Ethosight to dynamically apply post-processing phases that further refine the model's predictions.
\end{itemize}

\subsubsection{Evaluation Metrics and Results}


\begin{table}[ht]
    \centering
    \begin{tabular}{l c}
        \hline
        \textbf{Metric} & \textbf{Score} \\
        \hline
        Accuracy & 92.81\% \\
        Precision & 92.81\% \\
        Recall & 100\% \\
        F1 Score & 96.27\% \\
        Top-1 Accuracy & 25.15\% \\
        Top-5 Accuracy & 52.10\% \\
        Total Predictions & 167 \\
        \hline
    \end{tabular}
    \caption{Ethosight Evaluation Metrics for Multi-class Classification}
    \label{table:eval_metrics}
\end{table}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\columnwidth]{images/roc.png}
    \caption{ROC Curve1 - Ethosight Without Semantic Label Expansion}
    \label{fig:roc}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\columnwidth]{images/ucfcrime_multiclass.png}
    \caption{Supervised Model Multiclass Accuracy Comparison of UCF Crime dataset}
    \label{fig:multiclassComparison}
\end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.96\columnwidth]{images/chart.png}
    \caption{Supervised Model Anomaly Detection UCF Crime dataset}
    \label{fig:rocComparison}
\end{figure}

As shown in figures \ref{fig:multiclassComparison} and  \ref{fig:rocComparison}, initial testing of Ethosight zero-shot performance on the UCF Crime database does not achieve state-of-the-art performance when compared to supervised models. However, even at the current accuracy levels, Ethosight's ability to continuously and cumulatively learn and produce increasingly more accurate models may help narrow this performance gap. It should also be noted that, due to time constraints, these baseline numbers do not yet include the full performance expected from Ethosight's full capabilities. 

Due to the lack of datasets for detecting nuanced health, safety, and security related events and behaviors from single images, we are also releasing a new dataset containing 20 classes of interest including child in danger [figure: \ref{fig:kitchenaccident_event}].

\begin{figure}[ht]
\centering
\includegraphics[width=0.45\textwidth]{images/kitchenaccident.png}
\caption{Dangerous kitchen event detected by Ethosight.}
\label{fig:kitchenaccident_event}
\end{figure}

%\FloatBarrier

\begin{table}[ht]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Label} & \textbf{Affinity Score} \\ 
\hline
child in danger & 0.4346351623535156 \\ 
\hline
cooking & 0.26900413632392883 \\ 
\hline
burglary & 0.0736141949892044 \\ 
\hline
fire\_prevention & 0.07326945662498474 \\ 
\hline
gas\_leak\_detection & 0.06314415484666824 \\ 
\hline
repairing & 0.017247511073946953 \\ 
\hline
vomiting & 0.008393174037337303 \\ 
\hline
fire\_safety & 0.0065605794079601765 \\ 
\hline
decorating & 0.006369316019117832 \\ 
\hline
buying & 0.0054978723637759686 \\ 
\hline
peeping tom & 0.004484186880290508 \\ 
\hline
fire\_investigation & 0.0030823920387774706 \\ 
\hline
child abuse & 0.0020500756800174713 \\ 
\hline
oven & 0.0017948184395208955 \\ 
\hline
monitor & 0.0016760976286605 \\ 
\hline
\end{tabular}
\caption{Kitchen Event Labels and Affinity Scores}
\label{table:2}
\end{table}


Ethosight is an open source project and all code, data, and other digital artifacts are available as open source under the Apache 2.0 license.


==> sections/acknowledgements.tex <==
\subsubsection{Acknowledgements}
We express our gratitude to Cisco and Cisco Research, for providing the funding and resources for this work. Their support has been instrumental in driving our research forward.

We extend special thanks to the Meta team for their exceptional work on and open-source release of ImageBind and many other AI projects. Their contribution to the field has been invaluable and served as a pivotal resource in our project.

Our sincerest thanks to the broader community of researchers, developers, and enthusiasts whose interest in and feedback on our work has continually motivated us to improve and innovate.

==> sections/multimodalEmbedding.tex <==
\section{Multimodal Embedding}

A critical component of the Ethosight system is its incorporation of multimodal embeddings, facilitated through the application of Imagebind. Developed by the Meta team, this sophisticated multimodal model is instrumental in embedding a diverse array of data types — such as text, depth, heatmap, audio, inertial measurement unit (IMU) data, and images or videos — within a unified, cohesive framework. Imagebind is designed to learn and capture the subtle interrelationships between these diverse modalities, thereby forming a comprehensive representation of intricate data and events.

Ethosight utilizes Imagebind to generate new embeddings for novel labels and multimedia inputs. The resulting embeddings represent a combination of visual, auditory, textual, spatial, and situational data, providing a multi-faceted representation of complex scenarios.

The strengths of Ethosight lie in its effective utilization of the multimodal embeddings provided by Imagebind, its robust reasoning capabilities, and its implementation of localized label affinities. These attributes enable Ethosight to efficiently detect a wide spectrum of events, behaviors, and objects, and translate these detections into actionable insights.

The multimodal embeddings from Imagebind contribute to a comprehensive interpretation of diverse data modalities within Ethosight, aligning with local label affinities. The combination of these context-sensitive embeddings with the system's reasoning capabilities enhances Ethosight's functionality, enabling it to provide swift and relevant responses to a wide array of scenarios.

Another significant advantage of Ethosight is its compatibility with large-scale vision-language models like CLIP. This compatibility, along with the versatility of Imagebind, eliminates the need for specific training data, facilitating efficient adaptation to a multitude of contexts and challenges.

The integration of Imagebind's multimodal embeddings has proven to be highly effective for Ethosight, particularly in providing real-time actionable insights across various settings. The system has been successfully applied in areas like content moderation, sentiment analysis, and potential risk detection, emphasizing the importance of multimodal embeddings in the detection of events, behaviors, and objects. The conjunction of Imagebind and Ethosight illustrates the potential of multimodal embeddings in the development of adaptable and robust AI systems.

==> sections/userInteraction.tex <==
\section{User Interaction}
Ethosight is a pioneering application that fully leverages the Cisco open-source Deep Vision \cite{DeepVision} hybrid AI framework. The system allows users to effortlessly integrate cameras and other sensors, access analytics on multiple dashboards, and receive alerts through SMS or email via an intuitive, unified interface.

A notable feature of Ethosight's use of the Deep Vision framework is the integration of natural language processing (NLP) capabilities via the Deep Vision RecallM \cite{kynoch2023recallm} application. By harnessing the power of large language model (LLM) APIs such as ChatGPT and LangChain, Ethosight captures user intent and integrates it into the system's iterative reasoning loop which also supports reasoners to be integrated via a common interface. This process tailors the generation of personalized analytics to user specifications, whereby relevant labels (and their affinity scores) can both be generated automatically and driven by user questions.

Ethosight's ability to combine various reasoning components and unique knowledge representation from the Deep Vision system enhances its zero-shot video analytics capabilities. Through the amalgamation of natural language input and iterative reasoning, Ethosight can adapt to dynamic user requirements, significantly improving system utility and flexibility.

Ethosight, in conjunction with the Deep Vision framework, serves not just as a real-time analytics tool, but also as a platform for continued research and development. The system's compatibility with LLM APIs and the Deep Vision hybrid AI framework creates an interactive and user-friendly environment that encourages ongoing innovation, paving the way for future advancements in video analytics and real-time decision-making capabilities.

Ethosight's user-friendly interface, zero-shot video analytics, broad sensor integration capabilities, and potential for user customization make it adaptable to a range of applications. This design facilitates the delivery of sophisticated analytics in a user-friendly manner.

In conclusion, Ethosight marks a significant step forward within the Deep Vision framework. It enhances the efficiency and accessibility of AI systems by enabling user interaction through natural language inputs and providing real-time, personalized analytics, offering substantial potential for a variety of practical applications.

